SpaMEM: Benchmarking Dynamic Spatial Reasoning via Perception-Memory Integration in Embodied Environments

Multimodal large language models (MLLMs) have advanced static visual--spatial reasoning, yet they often fail to preserve long-horizon spatial coherence in embodied settings where beliefs must be continuously revised from egocentric observations under environmental change. We introduce SpaMEM (Spatial Memory from Action Sequences), a large-scale diagnostic benchmark that isolates the mechanics of spatial belief evolution via action-conditioned scene transformations (spawn, place, remove) over long interaction horizons. SpaMEM is built on a physically grounded dataset with 10,601,392 high-fidelity images across four modalities (RGB, depth, instance, semantic segmentation), collected from 25,000+ interaction sequences in 1,000 procedurally generated houses. We formalize embodied spatial reasoning as a three-level hierarchy with 15 diagnostic tasks: Level 1 measures atomic spatial perception from single observations; Level 2 probes temporal reasoning with oracle textual state histories to factor out perceptual noise; and Level 3 requires end-to-end belief maintenance from raw visual streams under the same task dimensions. We further evaluate both short-term (step-wise) updates and long-term (episodic) reconstruction. Benchmarking representative open-source VLM families reveals a consistent stacked bottleneck: coordinate-consistent grounding remains a hard ceiling, and the sharp collapse from Level 2 to Level 3 exposes a pronounced symbolic scaffolding dependency, where models succeed with text-based bookkeeping but struggle to sustain robust visual memory. SpaMEM provides a granular diagnostic standard and motivates explicit mechanisms for state representation, belief revision, and long-horizon episodic integration. A subset of SpaMEM is publicly available at https://huggingface.co/datasets/mill-ct-liao/SpaMEM.

==> sec/dataanalysis.tex <==
\section{Dataset Statistics and Scene Dynamics}
\label{sec:dataset_stats}

To rigorously evaluate long-horizon spatial memory, the SpaMEM dataset encompasses a massive and highly dynamic interaction space. As summarized in Table~\ref{tab:dataset_stats}, we generated the benchmark across \textbf{1,000 unique procedural houses} leveraging the ProcTHOR environment, meticulously recording multimodal observations including RGB, depth, instance, and semantic segmentation masks. Factoring in 16 distinct viewpoints (8 azimuthal angles $\times$ 2 heights) per state change, the dataset yields a total of \textbf{10,601,392 high-fidelity frames}. This scale offers the visual and geometric redundancy necessary to diagnose the ``Space-Time Dissonance'' observed in our experiments.

\noindent\textbf{Action Distribution and Causal Evolution.} 
The environment evolves through \textbf{33,220 discrete action steps} (see Fig.~\ref{fig:dataset_stats}, Left). The distribution is strategically designed to evaluate belief evolution: \textit{Spawn} (14,536 instances) and \textit{Place} (12,540 instances) operations dominate the sequences, gradually increasing the scene's geometric complexity and clutter. Meanwhile, \textit{Remove} actions (6,144 instances) explicitly test the models' capacity for belief revision and ``perceptual overwriting''. This action-conditioned dynamic evolution effectively shatters the static co-occurrence biases prevalent in traditional embodied benchmarks.

\noindent\textbf{Semantic and Geometric Diversity.}
To prevent models from exploiting semantic priors, SpaMEM features a rich taxonomy of \textbf{103 unique object types} interacting with \textbf{22 diverse receptacle types}. As illustrated in Fig.~\ref{fig:dataset_stats} (Bottom), we observe a persistent scale-dependent reliability gap, where high-volume objects are more easily grounded, whereas fine-grained or thin items such as \textit{Pencils} and \textit{Forks} represent a significant ``perceptual blindspot'' due to tokenization bottlenecks.

\noindent\textbf{Receptacle Bias and The Occlusion Challenge.}
An analysis of interaction frequency (Fig.~\ref{fig:dataset_stats}, Right) reveals that \textbf{Drawer} is the most frequently interacted container, appearing in 31,029 action steps. The prevalence of constrained-volume receptacles—including \textit{Shelves} (18,621) and \textit{Dressers} (6,275)—forces models to maintain robust episodic memory, as target objects frequently break line-of-sight. This contrasts with open-surface receptacles like \textit{Dining Tables} (15,695) or \textit{Beds} (9,246), where visual saliency is higher but geometric reasoning requirements are lower.

\input{table/spamen\_stats.tex} 

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figure/data_analysis/spamem_statistics.png}
  \caption{\textbf{SpaMEM Dataset Statistics.} (Left) Action distribution showing the balance between scene population and manipulation. (Right) Top-8 receptacle interaction frequency, highlighting the dominance of occluding containers like \textit{Drawers}. (Bottom) Top-15 object frequency distribution across the 103 unique categories, demonstrating semantic and scale diversity.}
  \label{fig:dataset_stats}
\end{figure}

==> sec/datageneration.tex <==
\section{Data Generation Pipelines}
\label{sec:data_generation}

To construct a large-scale, physically-grounded dataset for spatial reasoning and long-term memory evaluation, we developed an automated pipeline leveraging Large Language Models (LLMs) to orchestrate interactions within the ProcTHOR-10K environment \cite{deitke2022procthor}. Our framework balances high-level semantic reasoning with low-level physical constraints to ensure scene diversity and structural integrity.

\subsection{Structured Scene Representation: The World Graph}
Rather than providing raw point clouds or voxels to the decision-making agent, we abstract the 3D environment into a hierarchical \textit{World Graph} $\mathcal{G}$. For each room $\mathcal{R}_i$, the graph records:
\begin{itemize}
    \item \textbf{Receptacles:} Objects with containment properties (e.g., \textit{Cabinet}, \textit{Table}). For each receptacle, we calculate the Axis-Aligned Bounding Box (AABB) to estimate the available surface area $A_{free}$ in $cm^2$.
    \item \textbf{Object Hierarchy:} A set of parent-child relations $\mathcal{E} = \{(o_j, r_k)\}$ where object $o_j$ is supported by receptacle $r_k$. 
    \item \textbf{Spatial Attributes:} 3D coordinates, rotation, and semantic categories for every instance.
\end{itemize}
This structured representation allows the LLM to perform high-level reasoning over the spatial layout without the overhead of processing raw visual features during the planning stage.

\subsection{LLM-Guided Interaction Policy}
We employ \textbf{Qwen2.5-7B-Instruct} as a centralized reasoning engine to generate sequences of environment-modifying actions. The agent operates on a discrete action space $\mathcal{A} = \{spawn, place, remove\}$. 
To maintain realism, the agent is constrained by a specific set of small, pickable assets (e.g., \textit{Apple}, \textit{CellPhone}, \textit{Mug}) and instructed to avoid unstable or illogical placement targets such as \textit{Toilets} or \textit{Floor}. The decision process follows a "Think-and-Act" cycle: the LLM receives the current state of $\mathcal{G}$ and outputs a JSON-formatted command specifying the target object and the destination receptacle.

\subsection{Physically-Grounded Object Placement}
To bridge the gap between LLM text output and the 3D simulator, we implement a \textit{Smart Placement} heuristic. When an action involves placing an object $o$ onto a receptacle $r$, the system invokes a spatial search:
\begin{equation}
    P_{new} = \text{find\_smart\_position}(o, r, \mathcal{H})
\end{equation}
where $\mathcal{H}$ represents a set of category-specific heuristics (e.g., \textit{sink\_min} and \textit{hover\_max} parameters). 
For enclosed receptacles like \textit{Fridges} or \textit{Drawers}, the system automatically executes a pre-action \texttt{OpenObject} command, followed by a point-cloud-based search for valid coordinates above the interior shelves. If the initial placement triggers a physics collision, a recovery loop is initiated, prompting the LLM to suggest an alternative location or object.



\subsection{Multimodal Data Acquisition}
For every successful environment modification, we capture comprehensive multimodal snapshots from multiple viewpoints.
\begin{itemize}
    \item \textbf{Multi-view Coverage:} The agent teleports to 8 azimuthal angles ($0^\circ$ to $315^\circ$) and two camera heights (standing and crouching) to capture the target interaction from 16 distinct perspectives.
    \item \textbf{Rich Annotations:} Each viewpoint generates an RGB image, a depth map, and pixel-aligned instance/semantic segmentation masks. 
    \item \textbf{Spatial Metadata:} We log the 6-DOF camera pose, 2D/3D bounding boxes, and the updated World Graph, facilitating the training of models on tasks requiring precise spatial localization and long-term memory.
\end{itemize}

\subsection{Scalable Parallel Execution}
The generation process is parallelized across multiple worker processes to maximize throughput. Each worker manages an independent AI2-THOR instance, while a single GPU-accelerated server handles centralized LLM inference to minimize VRAM fragmentation. To ensure long-term stability, workers undergo a "soft reset" every five houses, clearing accumulated Unity engine artifacts and memory leaks. This architecture allowed us to simulate interactions across 700 unique procedural houses, resulting in a dataset of over 25,000 high-fidelity interaction sequences.

==> sec/spamem.tex <==
\section{SpaMEM}
\label{sec:framework}

\subsection{Evaluation Framework}
\label{subsec:eval_framework}

\paragraph{Overview.}
We introduce \textbf{SpaMEM} (\textbf{Spa}tial \textbf{M}emory), a hierarchical evaluation framework for diagnosing
(1) spatial grounding from instantaneous perception and
(2) temporal stability of world-state memory in embodied settings.
As illustrated in Fig.~\ref{fig:framework}, SpaMEM separates interaction into two explicit operating modes:
\textit{(i) Update Mode}, where the model \emph{reads} the current observation and \emph{updates} its internal belief state,
and \textit{(ii) Answer Mode}, where the model \emph{retrieves} information from the accumulated belief state to answer controlled spatial queries.
This separation turns spatial reasoning into a traceable process of \emph{state update} $\rightarrow$ \emph{state retrieval} $\rightarrow$ \emph{question answering} over time.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figure/main/framework.pdf}
\vspace{-18pt}
\caption{
\textbf{SpaMEM evaluation framework (Update and Answer Modes).}
At timestep $t$, the model observes a perceptual state $O_t$ (e.g., RGB, depth, instance, semantic) and a symbolic spatial state $S_t^{\ast}$ (e.g., topology clusters and 3D metadata).
\textbf{Update Mode:} the model reads $(O_t, S_t^{\ast})$ to update a spatial belief graph from $G_{t-1}$ to $G_t$.
\textbf{Answer Mode:} SpaMEM issues a query $q_t$ to retrieve from $G_t$ and produce an answer.
The probing protocol evaluates \textit{short-term} step-wise memory (queries during the episode) and \textit{long-term} episodic memory (queries only at $t = T$).
}
\vspace{-8pt}
\label{fig:framework}
\end{figure}

\paragraph{Framework pipeline.}
At each timestep $t$, the model receives two synchronized representations of the scene:
a perceptual state $O_t$ (raw visual observations and pixel-level cues) and a symbolic spatial state $S_t^{\ast}$ (structured entities and relations). 
In \textbf{Update Mode}, the model \emph{reads} $(O_t, S_t^{\ast})$ to incrementally update its latent world representation, formalized as a belief graph $G_t$ capturing entities (objects\slash receptacles) and their spatial relations.
In \textbf{Answer Mode}, SpaMEM injects a spatial query $q_t$; the model must \emph{retrieve} the relevant facts from $G_t$
and \emph{answer} with a verifiable output.
Crucially, SpaMEM does not assume the model exposes $G_t$ explicitly---we probe it through controlled retrieval questions.

\paragraph{Level 1: static spatial perception (L1).}
L1 benchmarks spatial grounding from a single timestep ($T{=}0$).
Tasks are restricted to a \emph{topology cluster}---a localized set of objects attached to a receptacle within one observation.
L1 measures recognition, 2D localization, depth/proximity estimation, relative-direction reasoning, and counting,
establishing a perception baseline before temporal updates are introduced.

\paragraph{Level 2: text-conditioned temporal memory (L2).}
L2 evaluates temporal reasoning over an episode $t{=}0\ldots T$ under \emph{oracle history}:
ground-truth textual summaries of past states are provided together with the current observation.
This setting assumes perfect historical perception, isolating the model's ability to update and query a consistent belief state over time
(e.g., lifespan grounding, trajectory reasoning, and state-difference inference) while minimizing accumulated recognition noise.

\paragraph{Level 3: visual-conditioned temporal memory (L3).}
L3 removes textual history and provides only a chronological stream of visual observations (with timestamps).
This is the most realistic end-to-end setting: the model must rely on visual evidence alone to maintain $G_t$ and answer spatio-temporal queries.

\paragraph{Temporal probing paradigms.}
For L2 and L3, we adopt two probing modes aligned with Fig.~\ref{fig:framework}.
\emph{Short-term (immediate)} probing issues queries step-wise ($t{-}1 \rightarrow t$) across the episode, assessing incremental updates and working-memory stability.
\emph{Long-term (episodic)} probing issues queries only at $t{=}T$, requiring retrieval over the full horizon $[0,T]$ and revealing long-horizon forgetting.

\paragraph{Diagnostic perspective.}
This three-level, two-paradigm design diagnoses failures in
(i) instantaneous spatial grounding (L1),
(ii) step-wise belief updates (short-term),
and (iii) long-horizon episodic integration (long-term).
% =========================================================
% Level 1
% =========================================================
\subsection{Level 1: Static Spatial Perception}
\label{subsec:l1_static_perception}

\paragraph{Task scope.}
L1 evaluates spatial understanding on individual frames within a topology cluster.
We decompose static perception into five dimensions.

\paragraph{Semantic object recognition (SOR).}
The model predicts the set of unique object categories within the cluster.
We report the $F_1$ score between predicted set $S_p$ and ground-truth set $S_g$:
\begin{equation}
\label{eq:l1_f1}
F_1 = \frac{2PR}{P+R}, \quad
P = \frac{|S_p \cap S_g|}{\max(|S_p|,1)}, \quad
R = \frac{|S_p \cap S_g|}{\max(|S_g|,1)}.
\end{equation}

\paragraph{Visual grounding and localization (VGL).}
The model predicts 2D bounding boxes for objects.
We evaluate IoU and report mean IoU (mIoU):
\begin{equation}
\label{eq:l1_iou}
\text{IoU} = \frac{\text{Area}(B_p \cap B_g)}{\text{Area}(B_p \cup B_g)}.
\end{equation}

\paragraph{Depth and proximity estimation (DPE).}
Model estimates absolute distance $d$ (meters) to each object.
We report mean absolute relative error (AbsRel):
\begin{equation}
\label{eq:absrel}
\text{AbsRel} = \frac{1}{N} \sum_{i=1}^{N} \frac{|d_i^g - d_i^p|}{d_i^g}.
\end{equation}
We additionally compute Spearman's rank correlation ($\rho$) to evaluate depth-order consistency.

\paragraph{Relative spatial relationship reasoning (RSR).}
Given an anchor object, the model predicts its $k$ nearest neighbors and their relative directions.
We report Recall@k (typically $k{=}3$) for neighbor identification and direction accuracy for egocentric relations.

\paragraph{Categorical and instance counting (CC/IC).}
The model predicts counts $C$ of categories (CC) or instances (IC).
We report absolute error (AE) and mean absolute percentage error (MAPE):
\begin{equation}
\label{eq:mape}
\text{AE} = |C_g - C_p|, \quad
\text{MAPE} = \frac{1}{N}\sum_{i=1}^{N}\frac{|C_i^g - C_i^p|}{\max(C_i^g,1)}.
\end{equation}
For instance counting, we also report Acc@k, where $|C_g - C_p| \le k$ with $k \in \{0,1\}$.

% =========================================================
% Level 2
% =========================================================
\subsection{Level 2: Text-Conditioned Temporal Memory}
\label{subsec:l2_text_memory}

\paragraph{Setting.}
L2 evaluates temporal reasoning across $t{=}0 \ldots T$ while providing ground-truth textual summaries of historical states.
This setup isolates temporal reasoning by eliminating historical perception noise.

\paragraph{Semantic and inventory (SI).}
The model recalls object categories at a specified past step (SOR-M) or aggregates all categories observed throughout the episode (LOR).
Both are evaluated using the $F_1$ score in Eq.~\ref{eq:l1_f1}.

\paragraph{Spatio-temporal localization (STL).}
We evaluate 2D grounding over time (VGL-M) and temporal lifespan localization (TL).
VGL-M uses mIoU (Eq.~\ref{eq:l1_iou}); TL uses temporal IoU:
\begin{equation}
\label{eq:tiou}
\text{tIoU} =
\frac{\max(0,\min(p_{last},g_{last})-\max(p_{first},g_{first})+1)}
{\max(p_{last},g_{last})-\min(p_{first},g_{first})+1}.
\end{equation}

\paragraph{Relations and trajectory tracking (RT).}
We evaluate neighborhood relations (RSR-M) and migration-path reconstruction (STT).
STT is measured by normalized edit similarity:
\begin{equation}
\label{eq:nes}
\text{NES} = 1 - \frac{\text{ED}(P,G)}{\max(|P|,|G|,1)}.
\end{equation}

\paragraph{Event detection and state reconstruction (SED/CSR).}
Short-term event detection (SED) and cumulative state reconstruction (CSR) evaluate added and removed sets independently using the $F_1$ metric in Eq.~\ref{eq:l1_f1}.

% =========================================================
% Level 3
% =========================================================
\subsection{Level 3: Visual-Conditioned Temporal Memory}
\label{subsec:l3_visual_memory}

\paragraph{Setting.}
L3 removes textual summaries and provides only the chronological visual sequence $\{(I_0,t_0), \dots, (I_{T-1},t_{T-1})\}$.
All task dimensions and metrics remain identical to L2 to ensure controlled comparison; only the modality of historical context differs.

\paragraph{Semantic and inventory (SI).}
The model recalls categories at a specified past step (SOR-M) and aggregates all categories observed across the episode (LOR) using only visual evidence.
Evaluation follows Eq.~\ref{eq:l1_f1}.

\paragraph{Spatio-temporal localization (STL).}
The model localizes objects over time (VGL-M) and predicts temporal lifespans (TL) directly from visual sequences.
Metrics follow Eq.~\ref{eq:l1_iou} and Eq.~\ref{eq:tiou}.

\paragraph{Relations and trajectory tracking (RT).}
Neighborhood relations (RSR-M) and migration paths (STT) are inferred solely from visual input.
STT is evaluated with normalized edit similarity (Eq.~\ref{eq:nes}).

\paragraph{Event detection and state reconstruction (SED/CSR).}
Step-wise event detection and end-of-episode state reconstruction evaluate added and removed sets independently using the $F_1$ metric in Eq.~\ref{eq:l1_f1}.

==> spamem_rebuttal_eccv/table/tab_r1.tex <==
% Tab. A: comparison with prior dynamic-scene benchmarks.
% Two binary columns - both verified safe against backbite:
%  - JSON graph: no prior bench requires JSON scene graph output
%  - Sym->vis control: only ToS has partial (separate worlds)
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}
\caption{\textbf{What SpaMEM tests that prior dynamic-scene benchmarks
do not.}\,\textbf{Graph out}: model required to emit step-wise JSON
scene graph (vs.\ action/VQA/index outputs). \textbf{Sym$\to$vis
control}: paired oracle-text vs.\ raw-image evaluation on the
\emph{same} trajectory and queries. \textbf{$\checkmark^\sim$}: ToS
has paired text/vision worlds but on \emph{separate} environments
under active exploration.}
\label{tab:r1}
\scriptsize
\begin{tabular}{@{}l l c c@{}}
\toprule
\textbf{Benchmark} & \textbf{Scene dynamics} &
\shortstack{\textbf{Graph}\\\textbf{out}} &
\shortstack{\textbf{Sym$\to$vis}\\\textbf{control}} \\
\midrule
TIDEE        & Misplaced$\to$placed     & {\color{red}\ding{55}} & {\color{red}\ding{55}} \\
SGM          & Object move + add/remove & {\color{red}\ding{55}} & {\color{red}\ding{55}} \\
DSI-Bench    & Continuous motion        & {\color{red}\ding{55}} & {\color{red}\ding{55}} \\
SAVVY-Bench  & Audio-visual events      & {\color{red}\ding{55}} & {\color{red}\ding{55}} \\
ENACT        & Predicate transitions    & {\color{red}\ding{55}} & {\color{red}\ding{55}} \\
FindingDory  & Pick-and-place           & {\color{red}\ding{55}} & {\color{red}\ding{55}} \\
ToS          & Object relocation        & {\color{red}\ding{55}} & {\color{green!50!black}\ding{51}}\textbf{$^\sim$} \\
\midrule
\textbf{SpaMEM (ours)} & \textbf{Spawn+Place+Remove} &
{\color{green!50!black}\ding{51}} & {\color{green!50!black}\ding{51}} \\
\bottomrule
\end{tabular}
\vspace{-12pt}
\end{table}


==> spamem_rebuttal_eccv/table/tab_r3.tex <==
% Tab. C: New baselines added in rebuttal — closed-source frontier,
% spatial-specific MLLM, and memory-augmented variant.
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.92}
\caption{\textbf{New baselines added in rebuttal.}\,L2$\to$L3 collapse
persists across model families and scales; SpatialBot's depth
pathway does not match generic VLMs' L2 reasoning. Memory-aug
recovers SOR-M identity but not grounding/tracking (VGL-M, STT
remain $\approx0$). SOR-M reported; full 15-metric in camera-ready.}
\label{tab:r3}
\scriptsize
\begin{tabular}{@{}l l c c c@{}}
\toprule
\textbf{Model} & \textbf{Type} &
\textbf{L2} & \textbf{L3} & \textbf{$\Delta$} \\
\midrule
\multicolumn{5}{l}{\emph{Closed-source / frontier-scale (R2)}} \\
GPT-5.4              & Closed   & 0.999 & 0.19 & 0.81 \\
GPT-4o               & Closed   & 0.989 & 0.14 & 0.85 \\
Qwen3-VL-235B-Inst.  & Open MoE & 0.996 & 0.17 & 0.83 \\
Qwen3-VL-32B-Inst.   & Open     & 0.997 & 0.29 & 0.70 \\
\midrule
\multicolumn{5}{l}{\emph{Spatial-specific MLLM (R2)}} \\
SpatialBot-3B (RGB-only) & Depth-aware & 0.46 & 0.00 & 0.46 \\
\midrule
\multicolumn{5}{l}{\emph{Memory-augmented (R1 sugg.~1)}} \\
InternVL3-8B + mem-aug & Oracle-summary aug.\ L3 & --- & \textbf{0.80} & --- \\
\midrule
InternVL3-8B (paper) & Open & 0.90 & 0.13 & 0.77 \\
\bottomrule
\end{tabular}
\vspace{-12pt}
\end{table}


==> spamem_rebuttal_eccv/table/tab_rB.tex <==
% Tab. C: New baselines added in rebuttal — closed-source frontier,
% spatial-specific MLLM, and memory-augmented variant.
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.92}
\caption{\textbf{New baselines added in rebuttal.}\,L2$\to$L3 collapse
persists across model families and scales; SpatialBot's depth
pathway does not match generic VLMs' L2 reasoning. Memory-aug
recovers SOR-M identity but not grounding/tracking (VGL-M, STT
remain $\approx0$). SOR-M reported; full 15-metric in camera-ready.}
\label{tab:rB}
\scriptsize
\begin{tabular}{@{}l l c c c@{}}
\toprule
\textbf{Model} & \textbf{Type} &
\textbf{L2} & \textbf{L3} & \textbf{$\Delta$} \\
\midrule
\multicolumn{5}{l}{\emph{Closed-source / frontier-scale (R2)}} \\
GPT-5.4              & Closed   & 0.999 & 0.19 & 0.81 \\
GPT-4o               & Closed   & 0.989 & 0.14 & 0.85 \\
Qwen3-VL-235B-Inst.  & Open MoE & 0.996 & 0.17 & 0.83 \\
Qwen3-VL-32B-Inst.   & Open     & 0.997 & 0.29 & 0.70 \\
\midrule
\multicolumn{5}{l}{\emph{Spatial-specific MLLM (R2)}} \\
SpatialBot-3B (RGB-only) & Depth-aware & 0.46 & 0.00 & 0.46 \\
\midrule
\multicolumn{5}{l}{\emph{Memory-augmented (R1 sugg.~1)}} \\
InternVL3-8B + mem-aug & Oracle-summary aug.\ L3 & --- & \textbf{0.80} & --- \\
\midrule
InternVL3-8B (paper) & Open & 0.90 & 0.13 & 0.77 \\
\bottomrule
\end{tabular}
\vspace{-12pt}
\end{table}


==> table/spamen_stats.tex <==
\begin{table}[t]
\centering
\caption{\textbf{SpaMEM Dataset Statistics.} Summary of the dataset scale, action distribution, and environmental diversity across 1,000 procedural houses.}
\label{tab:dataset_stats}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Metric} & \textbf{Count} & \textbf{Description} \\ \midrule
\textit{Scale \& Volume} &  &  \\
Total Procedural Houses & 1,000 & Diverse indoor layouts via ProcTHOR-10K \\
Total Interaction Steps & 33,220 & Total discrete environment state changes \\
Total Rendered Images & 10,601,392 & Multimodal: RGB, Depth, Instance, Semantic \\
Observation Viewpoints & 16 & 8 azimuthal angles $\times$ 2 camera heights \\ \midrule
\textit{Action Distribution} &  &  \\
Spawn Actions & 14,536 & Introduction of new objects to the scene \\
Place Actions & 12,540 & Manipulation and spatial relocation of objects \\
Remove Actions & 6,144 & Deletion of objects for belief revision testing \\ \midrule
\textit{Scene Diversity} &  &  \\
Unique Object Types & 103 & E.g., AlarmClock, ButterKnife, CellPhone \\
Unique Receptacle Types & 22 & E.g., Drawer, Chair, Shelf, Bed \\ \bottomrule
\end{tabular}
\end{table}
